TierBPF: Page Migration Admission Control for Tiered Memory via eBPF

Software-based memory tiering systems decide which pages to place on the slower or faster tier. However, they do not consider two important factors that greatly influence application performance: the size of the migrated pages, and the underlying hardware device and tiering topology. We introduce TierBPF, a software mechanism that can be plugged into existing memory tiering systems to take these factors into account, by making architecture-aware page admission decisions. TierBPF is implemented as a set of eBPF hooks, allowing users to define their custom policies. In order to make its decisions, TierBPF utilizes a lightweight tracking mechanism for page profiling which is not dependent on the application's working set size. TierBPF, integrated into three memory tiering systems and evaluated with 17 workloads, achieves geomean throughput gains of up to 15.9% with improvements of up to 75% for individual workloads.

==> table/table_tlb_miss.tex <==
\begin{table}[t]
\centering
\small
\caption{L2 DTLB misses per 1K instructions on the PMEM platform. MEMTIS's 4\,KB splitting incurs the highest TLB miss rates; \name's mTHP splitting reduces TLB overhead.}
  \vspace{-10pt}

\label{tab:tlb_miss}
\begin{tabular}{lcccc}
\toprule
\textbf{Workload} & \textbf{AutoNUMA} & \textbf{\name} & \textbf{MEMTIS} \\
\midrule
MG.D & 0.12 & 0.18 & 0.21 \\
 LU.D & 2.22 & 2.90 & 3.26 \\
\bottomrule
\end{tabular}
  \vspace{-10pt}

\end{table}


==> template/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.16   Emergency release: fixes a typo in the code.

Version 2.15   Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> text/ack.tex <==
\begin{comment}
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}
\end{comment}

==> text/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

%Modern datacenter applications demand ever-larger memory capacities. To meet this demand without proportional cost increases, operators deploy \emph{tiered memory} systems that combine fast but expensive local DRAM with slower but cheaper memory technologies. The operating system manages these tiers transparently through \emph{page migration}: promoting hot pages to fast-tier memory and demoting cold pages to slow-tier memory~\cite{maruf2023tpp, vuppalapati2024colloid, xiang2024nomad}.

Modern datacenter workloads require memory capacities that exceed what can be economically provisioned with DRAM alone. To bridge this gap, operators deploy tiered memory architectures that pair fast, capacity-limited local DRAM with slower, higher-capacity memory technologies. The operating system (OS) manages these heterogeneous tiers transparently via page migration, dynamically promoting frequently (or recently) accessed pages to fast-tier memory and demoting infrequently used pages to slower tiers~\cite{maruf2023tpp, vuppalapati2024colloid, xiang2024nomad,10.1145/3676642.3736119,eurosys24:mtm}.

%Today's slow-tier memory is no longer a single technology. CXL-attached DRAM uses a PCIe-based interconnect， Intel Optane PMEM connects through the DDR bus, and emerging technologies such as CXL-attached flash~\cite{} and disaggregated memory pools~\cite{} continue to expand the design space. These technologies differ not only in latency and bandwidth, but also in fundamental properties such as duplex mode, persistence, and cache coherence. As a result, the same migration policy can yield very different performance outcomes depending on the underlying hardware. A promotion strategy that improves throughput on a CXL platform may be counterproductive on Optane, or vice versa (\S\ref{subsec:mot-arch}). Yet the tiering systems deployed today are tightly coupled to specific assumptions about the slow tier. They hard-code a single migration policy into the kernel, leaving operators no way to adapt when the hardware changes. As memory architectures continue to diversify, this lack of flexibility becomes a growing problem.

Slow-tier memory is no longer defined by a single technology. CXL-attached memory expansion connects over a PCIe link, Intel Optane PMEM is integrated via the DDR bus, and emerging substrates—such as CXL-attached flash~\cite{} and disaggregated memory pools~\cite{}—further broaden the design space. These platforms differ not only in latency and bandwidth, but also in architectural properties such as duplex mode, persistence, and cache coherence. As a result, migration policies interact differently with each memory substrate: a policy that improves performance on a CXL-based memory expansion may have little benefit—or even incur overhead—on persistent memory-based platforms (\S\ref{subsec:mot-arch}). However, existing tiered memory systems are typically designed around a fixed set of assumptions about the slow tier, embedding a single migration policy into the kernel. As memory technologies continue to diversify, this tight coupling limits the effectiveness of page migration across platforms.

%Beyond the choice of migration policy, the \emph{granularity} of migration also matters. Most production systems enable Transparent Huge Pages (THP), allocating memory in 2\,MB pages to reduce TLB miss overhead. However, page migration and THP interact poorly. When the kernel migrates a 2\,MB THP, it must copy the entire page, even if only a small fraction of its subpages are frequently accessed. This wastes migration bandwidth and occupies scarce fast-tier capacity with cold data. The alternative, splitting the THP into 512 base pages and migrating only the hot ones, destroys the TLB coverage that huge pages provide. Linux 6.8 introduced multi-size THP (mTHP), which supports intermediate page sizes from 16\,KB to 1\,MB, but only for \emph{allocation}. No existing system uses mTHP sizes when \emph{migrating} pages between memory tiers. This leaves a middle ground entirely unexplored: splitting a 2\,MB THP into an intermediate mTHP size (e.g., 64\,KB or 256\,KB) that captures the hot region without sacrificing all TLB benefits.


Beyond the choice of migration policy, the granularity of migration is equally critical. Most production systems enable Transparent Huge Pages (THP), allocating memory in 2\,MB pages to reduce TLB miss overhead. However, page migration interacts poorly with THP. When the kernel migrates a 2\,MB THP, it must copy the entire page, even if only a small subset of its constituent base pages are frequently accessed. This behavior wastes migration bandwidth and fills scarce fast-tier capacity with cold data. Splitting the THP into 512 base pages and migrating only the hot ones avoids this waste, but at the cost of destroying the TLB coverage that huge pages provide. Linux 6.8 partially addresses this tension by introducing multi-size THP (mTHP), which supports intermediate page sizes from 16\,KB to 1\,MB, but only at \emph{allocation} time. No existing system exploits mTHP sizes during \emph{migration} across memory tiers. Consequently, a promising middle ground remains unexplored: dynamically splitting a 2\,MB THP into an intermediate mTHP size (e.g., 64\,KB or 256\,KB) that captures hot regions while retaining much of the TLB benefit of huge pages.

\begin{comment}
Exploiting this middle ground is not straightforward.
Two challenges stand in the way.
First, the right mTHP size is not static.
Under low bandwidth contention, keeping pages at 2\,MB is optimal because TLB coverage dominates.
Under high bandwidth contention, which is common in multi-tenant cloud environments, smaller mTHP sizes are preferable because they reduce bandwidth waste and fast-tier capacity consumption per migration (\S\ref{subsec:mot-contention}).
A system must therefore adapt its page size selection dynamically based on runtime conditions.
\end{comment}

Exploiting this middle ground, however, is fundamentally challenging. Two obstacles stand in the way. First, the optimal mTHP size is inherently dynamic. When migration bandwidth is unconstrained, preserving 2\,MB pages is preferable, as TLB coverage dominates performance. In contrast, under high migration bandwidth contention—common in multi-tenant cloud environments—smaller mTHP sizes are more effective, as they sharply reduce both wasted migration traffic and fast-tier capacity consumption per promotion (\S\ref{subsec:mot-contention}). A  practical system must therefore adapt page-size decisions to evolving runtime conditions rather than rely on a static granularity choice.

\begin{comment}
Second, different memory architectures demand different migration strategies.
CXL memory uses full-duplex links where reads and writes proceed on independent channels, while Optane PMEM uses half-duplex DDR where reads and writes share the same bus.
This architectural difference means that a migration policy beneficial on one platform can hurt performance on another (\S\ref{subsec:mot-arch}).
For example, on a CXL system where the memory traffic is read-dominant, selectively holding back write-heavy pages from promotion can improve bandwidth utilization by keeping the full-duplex channels balanced.
The same policy on Optane would merely prevent hot pages from reaching fast memory, with no bandwidth benefit. Yet existing tiering systems (e.g., AutoNUMA~\cite{autonuma}, TPP~\cite{maruf2023tpp}, MEMTIS~\cite{lee2023memtis}, Colloid~\cite{vuppalapati2024colloid}, Nomad~\cite{xiang2024nomad} and HybridTier~\cite{10.1145/3676642.3736119}) all apply a single, architecture-agnostic migration policy.
\end{comment}

Second, migration policies must be architecture-aware. Emerging memory platforms differ in how migration traffic interacts with hardware resources. CXL memory employs full-duplex links, allowing reads and writes to proceed on independent channels, whereas Intel PMEM relies on half-duplex DDR interfaces where reads and writes contend for the same bus. As a result, a migration strategy that improves performance on one architecture can degrade it on another (\S\ref{subsec:mot-arch}). For example, on a read-dominant CXL system, deliberately suppressing the promotion of write-heavy pages balances bidirectional bandwidth utilization and improves effective throughput. Applying the same policy on PMEM yields no such benefit; it merely delays the placement of hot pages into fast memory. Despite these fundamental differences, existing tiering systems—including AutoNUMA~\cite{autonuma}, TPP~\cite{maruf2023tpp}, MEMTIS~\cite{lee2023memtis}, Colloid~\cite{vuppalapati2024colloid}, Nomad~\cite{xiang2024nomad}, and HybridTier~\cite{10.1145/3676642.3736119}—all hard-code a single, architecture-agnostic migration policy.

% TODO: Consider adding a figure here that provides a high-level illustration
% of the FlexTier approach (e.g., a before/after comparison of 2MB migration
% vs. mTHP-aware migration), if space permits.

%These challenges call for flexibility in both migration granularity and migration strategy. Such flexibility that cannot be achieved by hard-coding a single policy into the kernel. We observe that eBPF, which allows safe, verified programs to run inside the kernel without recompilation, is well-suited for this task. By placing programmable hooks on the kernel's migration path, we can decouple \emph{what} to migrate and \emph{at what granularity} from the kernel's migration mechanism itself, adapting policy to the workload, the runtime environment, and the hardware.

These challenges demand flexibility in both migration granularity and migration strategy—flexibility that cannot be achieved by hard-coding a single policy into the kernel. We observe that eBPF, which enables safe, verified programs to execute inside the kernel without recompilation, provides a natural substrate for such adaptability. By inserting programmable hooks along the kernel’s migration path, we cleanly decouple \emph{what} to migrate and \emph{at what granularity} from the migration mechanism itself. This separation allows migration policy to evolve dynamically with the workload, runtime conditions, and underlying hardware, without sacrificing safety or deployability.


\begin{comment}
In this paper, we present \name, an eBPF-based memory tiering system that makes THP migration both granularity-aware and architecture-aware.
\name introduces three key techniques.
(1)~\emph{Contention-aware mTHP splitting}: when slow-tier bandwidth is under pressure, \name splits 2\,MB THPs into the largest mTHP size that still captures the hot subpage region, preserving TLB coverage while avoiding bandwidth waste.
When bandwidth contention is low, pages remain at 2\,MB.
(2)~\emph{Architecture-aware migration admission}: on CXL platforms, \name evaluates each page's read/write ratio against real-time CXL traffic before allowing page migration to determine whether a page should be migrated or not. This hook is a no-op on half-duplex architectures.
(3)~\emph{Lightweight eBPF-based profiling}: \name processes hardware memory access samples (AMD IBS / Intel PEBS) entirely in-kernel via eBPF programs, avoiding the context switches and data copies of user-space profiling.
A compact global subpage histogram (4\,KB per process) replaces per-page tracking structures that can grow to hundreds of megabytes, enabling low-overhead profiling regardless of working set size.
\end{comment}

In this paper, we present \name, an eBPF-based memory tiering system that makes THP migration both granularity-aware and architecture-aware. \name introduces three core techniques.
(1) Contention-aware mTHP splitting: when slow-tier bandwidth becomes constrained, \name selectively splits a 2\,MB THP into the largest mTHP size that still captures the hot subpage region, preserving most TLB coverage while eliminating wasted migration traffic. %When contention is low, pages remain intact at 2\,MB.
(2) Architecture-aware migration admission: on CXL platforms, \name evaluates each page’s read/write ratio against real-time CXL traffic and admits migration only when it improves bidirectional bandwidth utilization; on half-duplex architectures, this check becomes a no-op. 
(3) Lightweight eBPF-based profiling: \name processes hardware memory access samples entirely in-kernel using eBPF, avoiding the context switches and data copies of user-space profiling. A lightweight, compact global subpage histogram (4\,KB per process) replaces per-page tracking structures that can otherwise grow to hundreds of megabytes, enabling consistently low-overhead profiling independent of working set size.

%We evaluate \name on two diverse memory platforms (one with CXL memory expansion and the other with Intel PMEM) across representative memory-intensive workloads. 

We summarize the contributions as follows. 
%% TODO: Fill in final numbers after evaluation is complete.
%% Example: \name improves application performance by up to X\% compared to
%% the best prior system, while reducing migration bandwidth by Y\%.


\begin{itemize}
    \item We identify a fundamental lack of flexibility in existing memory tiering systems in the face of growing architectural diversity. In particular, we show that the interaction between THP and page migration, as well as migration admission control, has become a first-order bottleneck that cannot be addressed by static, kernel-hardcoded policies.  
    %With the emerging diversity across memory tiering architectures, we identify the necessity of bringing flexibility into memory tiering software system, especially in the interaction between THP and page migration, and page migration admission control. 
    %We identify the interaction between THP and page migration as a key inefficiency in tiered memory systems, and show that intermediate mTHP sizes can resolve the tension between migration precision and TLB coverage (\S\ref{sec:motivation}).

    \item We present \name, the first system to support mTHP-granularity page migration with dynamic, contention-aware granularity selection and architecture-aware migration admission. \name implements all migration policies as eBPF programs, requiring only minimal kernel changes and enabling rapid policy evolution without kernel recompilation   
    %We present \name, the first system to perform mTHP-granularity page migration with dynamic, contention-aware size selection and architecture-aware migration admission. All policies are implemented as eBPF programs, requiring minimal kernel changes and no kernel recompilation for policy updates (\S\ref{sec:key-ideas}--\S\ref{sec:design}).

    %\item We introduce a lightweight profiling approach that uses eBPF to process hardware samples in-kernel with a compact global subpage histogram, reducing profiling memory overhead from hundreds of megabytes to 4\,KB per process (\S\ref{subsec:profiling}).

    \item We evaluate \name on two different memory platforms—one based on CXL memory expansion and the other on Intel PMEM—and integrate \name with multiple existing memory tiering systems (\textcolor{red}{xxxxxxxx
}). Our results demonstrate that \name significantly improves both adaptability and performance across architectures, outperforming prior approaches under diverse workloads by \textcolor{red}{xxxxxx}.
    %We evaluate \name on two diverse memory platforms (one with CXL memory expansion and the other with Intel PMEM) and integrate it with xxxx memory tiering systems (xxxx). We demonstrate the great flexibility brought by xxxx, and outperforms by xxxx. 

\end{itemize}

